Hausdorff Point Convolution with Geometric Priors

Without a shape-aware response, it is hard to characterize the 3D geometry of a point cloud efficiently with a compact set of kernels. In this paper, we advocate the use of Hausdorff distance as a shape-aware distance measure for calculating point convolutional responses. The technique we present, coined Hausdorff Point Convolution (HPC), is shape-aware. We show that HPC constitutes a powerful point feature learning with a rather compact set of only four types of geometric priors as kernels. We further develop a HPC-based deep neural network (HPC-DNN). Task-specific learning can be achieved by tuning the network weights for combining the shortest distances between input and kernel point sets. We also realize hierarchical feature learning by designing a multi-kernel HPC for multi-scale feature encoding. Extensive experiments demonstrate that HPC-DNN outperforms strong point convolution baselines (e.g., KPConv), achieving 2.8% mIoU performance boost on S3DIS and 1.5% on SemanticKITTI for semantic segmentation task.

==> consistency.tex <==
\begin{figure*}[t]
	\begin{overpic}[width=0.9\textwidth,tics=5]{fig/Overview.png}
	\end{overpic}
	\caption{
		The consistency of 2D discrete convolution and Hausdorff convolution in geometric meaning. For comparing two shapes, the 2D discrete convolution uses the inner product approach, and the Hausdorff distance is adapted on 3D point clouds.}
	\label{fig:overview}
\end{figure*} 


==> kernelshape.tex <==
\begin{figure}[t]
	\centering
	\begin{overpic}
	[width=0.9\linewidth]{fig/Kernels/kernelshape.png}
	%%\caption{(a) Synthetic}
	\put(1,78){\small (a)}
	\put(56,78){\small (c)}
	\put(1,35){\small (b) }
	\put(56,35){\small (d) }
	\end{overpic}
	\caption{
		The generated basic geometric primitives in the neighborhood space (blue region): from (a) to (d) is the 3D sphere, 2D plane, 1D straight line and 0D center point, respectively.}
	\label{fig:kernelshape}
\end{figure} 


==> laserbeam.tex <==
\begin{figure}[t]
	\centering
	\begin{overpic}[width=0.4\textwidth]{fig/teaser.png}
	\end{overpic}
	\caption{
		A typical point cloud scene has data outliers and occluded data absence, resulting in incomplete local shapes with gaps... placeholder}
	\label{fig:teaser}
\end{figure} 

